Quasirandom additive sets and Cayley hypergraphs

We study the interplay between notions of quasirandomness for additive sets and for hypergraphs. In particular, we show a strong connection between the notions of Gowers uniformity in the additive setting and discrepancy-type measures of quasirandomness in the hypergraph setting. Exploiting this connection, we provide a long list of disparate quasirandom properties regarding both additive sets and Cayley-type hypergraphs constructed from such sets, and show that these properties are all equivalent (in the sense of Chung, Graham and Wilson) with polynomial bounds on their interdependences.

==> Towsner.tex <==
\appendix

\section{Towsner's results}

In this appendix we outline a proof of Towsner's Theorem on quasirandomness of any order~$d$ which obtains polynomial bounds.


Given a $k$-partite $k$-graph $F$ with vertex partition $X_1, \dots, X_k$ and some subset $I \subseteq [k]$ of the indices, we define the \emph{$I$-doubling} of $F$ to be the hypergraph $\db_I(F)$ obtained by taking two copies of $F$ and identifying the corresponding vertices in the classes $X_i$, for all $i \in I$.
More precisely, the vertex set of the $I$-doubling is
\begin{equation*}
    V(\db_I(F)) = Y_1 \cup \dots \cup Y_k \hspace{3mm} \text{where} \hspace{3mm} Y_i =
    \begin{cases}
        X_i & \text{ if } i \in I, \\
        X_i \times \{0, 1\} & \text{ if } i \notin I 
    \end{cases}
\end{equation*}
and its edge set is the collection of all $k$-sets of the form
$$\{x_i:\, i \in I\} \cup \{(x_j, a):\, j \in [k] \setminus I\},$$
where $a \in \{0, 1\}$ and $\{x_i:\, i \in [k]\}$ is an edge of $F$.

Starting with the $k$-partite hypergraph with $k$ vertices and a single edge, and then applying consecutively $\db_I$ for every $I \in \binom{[k]}{d}$ (in some arbitrary order), we get a $d$-linear $k$-graph we shall denote by $\M^{(k)}_{d}$.
One can think of this construction of $\M^{(k)}_{d}$ as encoding the applications of Cauchy-Schwarz needed in the proof that correctly counting $d$-linear $k$-graphs implies quasirandomness of order
$d$\footnote{An interesting way to formalize this idea is by considering the \emph{Cauchy-Schwarz tree} (as defined in \cite{GraphNorms}) associated with the cut involutions representing which vertices are fixed by each elementary doubling operation in the construction of $\M^{(k)}_{d}$.
We refer the reader to sections 3 and 5 of \cite{GraphNorms}.}.

The conjecture that $\M^{(k)}_{d}$ is complete for quasirandomness of order $d$ was later proven by Towsner \cite{SigmaAlgebrasHypergraphs} (using the framework of ultraproducts and graded probability spaces), who then obtained the main equivalence theorem for quasirandomness of any fixed order.
We reproduce his result below:

\begin{thm}
Let $1 \leq d < k$ be integers and let $H$ be a $k$-uniform hypergraph with edge density $\delta$.
Then the following properties are asymptotically equivalent:
\begin{itemize}
    \item[$(i)$] $H$ is quasirandom of order $d$: \hspace{2mm}
    $\| H - \delta \|_{\square^{k}_d} \leq c_1$
    \item[$(ii)$] $H$ correctly counts all $d$-linear hypergraphs:
    $$t(F, H) = \delta^{|F|} \pm c_2 |F| \hspace{5mm} \forall F \in \mathcal{L}^{(k)}_{d}$$
    \item[$(iii)$] $H$ has few copies of $M = \M^{(k)}_{d}$: \hspace{2mm}
    $t(M, H) \leq \delta^{|M|} + c_3$
    \item[$(iv)$] $H$ has small deviation with respect to $M = \M^{(k)}_{d}$:
    $$\mathbb{E}_{\xbf \in V(H)^{V(M)}} \Bigg[\prod_{e \in M} \big(H(\xbf_{e}) - \delta\big) \Bigg] \leq c_4$$
\end{itemize}
\end{thm}

Define the norm $\|\cdot\|_{\M^{(k)}_d}$ and the corresponding Cauchy-Schwarz type inequality.

The implication $(i) \Rightarrow (ii)$ follows from the same kind of argument we used before.
Moreover, since $\M^{(k)}_d$ is $d$-linear and $\|H\|_{\M^{(k)}_d} \geq \mathbb{E}[H] = \delta$, item $(iii)$ is a special case of property $(ii)$.

To prove $(iii) \Rightarrow (iv)$:
By the Cauchy-Schwarz inequality we see that $t(F, H) \leq \|H\|_{\M^{(k)}_d}^{|F|}$ for all $F \subseteq \M^{(k)}_d$, so
\begin{align*}
    t\big(\M^{(k)}_d, H + \delta\big) + t\big(\M^{(k)}_d, H - \delta\big)
    &\leq \sum_{F \subseteq \M^{(k)}_d} \|H\|_{\M^{(k)}_d}^{|F|} \big( \delta^{|\M^{(k)}_d| - |F|} + (-\delta)^{|\M^{(k)}_d| - |F|} \big) \\
    &= \big( \|H\|_{\M^{(k)}_d} + \delta \big)^{|\M^{(k)}_d|} + \big( \|H\|_{\M^{(k)}_d} - \delta \big)^{|\M^{(k)}_d|}.
\end{align*}
Using that $t(\M^{(k)}_d, H + \delta) \geq (2\delta)^{|\M^{(k)}_d|}$ we easily conclude.

To prove $(iv) \Rightarrow (i)$:
Take an edge $\tau_0 = \{v_1, \dots, v_k\} \in \M^{(k)}_d$.
From the construction of $M = \M^{(k)}_d$, one can show that there exist \emph{distinct} edges $\tau_D \in M \setminus \{\tau_0\}$, $D \in \binom{[k]}{d}$, such that $\{v_i:\, i \in D\} \subset \tau_D$ for all $D \in \binom{[k]}{d}$.

Define the functions $(f_{\sigma})_{\sigma \in M}$ by $f_{\tau_0} = f$,
$f_{\tau_D}(x_1, \dots, x_k) = u_D((x_i)_{i \in D})$
for all $D \in \binom{[k]}{d}$, and $f_{\sigma} \equiv 1$ for all other $\sigma \in M$.
Then
\begin{align*}
    \mathbb{E}_{x_1, \dots, x_k \in V} \Bigg[ f(x_1, \dots, x_k) \prod_{D \in \binom{[k]}{d}} u_D \big((x_i)_{i \in D}\big) \Bigg]
    &= \mathbb{E}_{\xbf \in V^{V(M)}} \Bigg[ f(\xbf_{\tau_0}) \prod_{D \in \binom{[k]}{d}} f_{\tau_D}(\xbf_{\tau_D}) \Bigg] \\
    &= \big\langle (f_{\sigma})_{\sigma \in \M^{(k)}_d} \big\rangle_{\M^{(k)}_d},
\end{align*}
which is at most $\|f\|_{\M^{(k)}_d}$.

The $k$-partite version of this result also holds, with the same bounds and essentially the same proof.


==> extensions.tex <==
\section{Possible extensions and limitations}
\label{sec:extensions}


\subsection{More general Cayley-type hypergraphs} \label{sec:general_Cayley}

While our choice of modeling an additive set $A$ by the hypergraph $\Gamma^{(k)}_A$ encoding its sum is quite natural, it is nevertheless somewhat arbitrary.
One could also think of different hypergraphs which encode this same set $A$ but making use of other linear forms.
In this subsection we will study to what extent the results obtained in Section~\ref{sec:set_hypergraph} depend on the choice of linear form.

We define a linear form $\phi: G^k \rightarrow G$ as any map of the form
$$(x_1, \dots, x_k) \,\mapsto\, \lambda_1 x_1 + \dots + \lambda_k x_k,$$
where $\lambda_1, \dots, \lambda_k$ are integers.
Since such forms are not necessarily symmetric in their variables, we will need to consider $k$-partite hypergraphs associated to them.

\begin{definition}
Given a linear form $\phi: G^k \rightarrow G$ and a set $A \subseteq G$, define the $k$-partite $k$-graph $\Gamma^{\phi}_A$ as follows:
each vertex class $V_i$, $1 \leq i \leq k$, is a copy of $G$ and $\{x_1, \dots, x_k\} \in \prod_{i\leq k} V_i$ is in $\Gamma^{\phi}_A$ iff $\phi(x_1, \dots, x_k) \in A$.
\end{definition}



\begin{thm} \label{thm:general_Cayley}
Let $G$ be a finite additive group and $A \subseteq G$ be a subset.
\begin{itemize}
    \item[$(i)$] If $A$ is $\varepsilon$-uniform of degree $d$, then for any $k \geq d+1$ and any linear form $\phi: G^k \rightarrow G$ the hypergraph $\Gamma^{\phi}_A$ is $\varepsilon'$-quasirandom of order $d$, with
    $$\varepsilon' = \varepsilon \Bigg( \prod_{i=1}^{d+1} \frac{|G|}{|\lambda_i G|} \Bigg)^{1/2^{d}}.$$
    \item[$(ii)$] Conversely, if $\phi: G^{d+1} \rightarrow G$ is surjective and $\Gamma^{\phi}_A$ is $\varepsilon$-quasirandom of order $d$, then $A$ is $\varepsilon'$-uniform of degree $d$, with $\varepsilon' = 2 \varepsilon^{1/2^{d+1}}$.
\end{itemize}
\end{thm}

Note the asymmetry in the conditions required for each item of this theorem:
for item $(i)$ we require the subgroups $\lambda_i G$ to not be much smaller than $G$ itself (otherwise our conclusion still holds but it is trivial), while for item $(ii)$ we instead require the linear form $\phi$ to be surjective.

After the proof of the theorem, we will show by way of examples that this asymmetry is in fact \emph{necessary}.
Indeed, even if the linear form $\phi: G^k \rightarrow G$ (or some restricted subform on $d+1$ variables) is surjective, the hypergraph $\Gamma^{\phi}_A$ of a very uniform set $A$ needs not be quasirandom;
and even if the subgroups $\lambda_i G$ are all `large', without surjectivity of $\phi$ we cannot conclude uniformity of $A$ from quasirandomness of $\Gamma^{\phi}_A$.

\begin{proof}[Proof of Theorem~\ref{thm:general_Cayley}]
$(i)$
We will first show the case when $k=d+1$, which says that
$$\|\Gamma^{\phi}_A - \delta\|_{\square^{d+1}_{d}} \leq \Bigg( \prod_{i=1}^{d+1} \frac{|G|}{|\lambda_i G|} \Bigg)^{1/2^{d}} \|A - \delta\|_{U^{d+1}}$$
for all linear forms
$\phi: (x_1, \dots, x_{d+1}) \mapsto \lambda_1 x_1 + \dots + \lambda_{d+1} x_{d+1}$.

Denote by $g := A - \delta$ the balanced function of $A$.
By Gowers-Cauchy-Schwarz we have
$$\|\Gamma^{\phi}_A - \delta\|_{\square^{d+1}_d}^{2^{d+1}} \leq \|\Gamma^{\phi}_A - \delta\|_{\oct^{d+1}}^{2^{d+1}}
= \mathbb{E}_{\xbf^{(0)}, \xbf^{(1)} \in G^{d+1}} \Bigg[ \prod_{\omega \in \{0, 1\}^{d+1}} g \bigg( \sum_{i=1}^{d+1} \lambda_i x_i^{(\omega_i)} \bigg) \Bigg].$$
Making the change of variables $y_i^{(0)} = \lambda_i x_i^{(0)}$, $y_i^{(1)} = \lambda_i x_i^{(1)}$ for $1 \leq i \leq d+1$, the expression above becomes
\begin{align*}
    &\mathbb{E}_{\ybf^{(0)}, \ybf^{(1)} \in \prod_{i=1}^{d+1} \lambda_i G} \Bigg[ \prod_{\omega \in \{0, 1\}^{d+1}} g\bigg( \sum_{i=1}^{d+1} y_i^{(\omega_i)} \bigg) \Bigg] \\
    &= \Bigg( \prod_{i=1}^{d+1} \frac{|G|}{|\lambda_i G|} \Bigg)^2 \mathbb{E}_{\ybf^{(0)}, \ybf^{(1)} \in G^{d+1}} \Bigg[ \mathbbm{1}_{\prod_i \lambda_i G}(\ybf^{(0)}) \,\mathbbm{1}_{\prod_i \lambda_i G}(\ybf^{(1)}) \prod_{\omega \in \{0, 1\}^{d+1}} g \big(\Sigma(\ybf^{(\omega)})\big) \Bigg].
\end{align*}
The last expectation can be written in two different but equivalent ways:
either as
\begin{equation*}
    \mathbb{E}_{\ybf^{(0)}, \ybf^{(1)} \in G^{d+1}} \Bigg[ \prod_{\omega \in \{0, 1\}^{d+1}} \mathbbm{1}_{\prod_i \lambda_i G}(\ybf^{(\omega)})\, g \big(\Sigma(\ybf^{(\omega)})\big) \Bigg]
    = \big\| \mathbbm{1}_{\prod_i \lambda_i G} \cdot \Gamma^{(d+1)}_g \big\|_{\oct^{d+1}}^{2^{d+1}},
\end{equation*}
or as $\big\langle (f_{\omega})_{\omega \in \{0, 1\}^{d+1}} \big\rangle_{\oct^{d+1}}$ where
$$f_{\omega} =
\begin{cases}
    \mathbbm{1}_{\prod_i \lambda_i G} \cdot \Gamma^{(d+1)}_g &\text{ if } \omega = 0^{d+1} \text{ or } 1^{d+1}, \\ 
    \Gamma^{(d+1)}_g &\text{ otherwise.}
\end{cases}$$
By Gowers-Cauchy-Schwarz we then obtain
\begin{align*}
    \big\| \mathbbm{1}_{\prod_i \lambda_i G} \cdot \Gamma^{(d+1)}_g \big\|_{\oct^{d+1}}^{2^{d+1}}
    &= \big\langle (f_{\omega})_{\omega \in \{0, 1\}^{d+1}} \big\rangle_{\oct^{d+1}} \\
    &\leq \big\| \mathbbm{1}_{\prod_i \lambda_i G} \cdot \Gamma^{(d+1)}_g \big\|_{\oct^{d+1}}^2 \|\Gamma^{(d+1)}_g\|_{\oct^{d+1}}^{2^{d+1}-2},
\end{align*}
from which we conclude
$\big\| \mathbbm{1}_{\prod_i \lambda_i G} \cdot \Gamma^{(d+1)}_g \big\|_{\oct^{d+1}} \leq \|\Gamma^{(d+1)}_g\|_{\oct^{d+1}}$.
Thus
$$\|\Gamma^{\phi}_A - \delta\|_{\square^{d+1}_d}^{2^{d+1}} \leq \Bigg( \prod_{i=1}^{d+1} \frac{|G|}{|\lambda_i G|} \Bigg)^2 \|\Gamma^{(d+1)}_g\|_{\oct^{d+1}}^{2^{d+1}},$$
which is precisely what we wanted
(recall that $\|\Gamma^{(d+1)}_g\|_{\oct^{d+1}} = \|A - \delta\|_{U^{d+1}}$).

If $k > d+1$, then we first separate the linear form $\phi$ into its part $\phi'$ which depends on the first $d+1$ variables and its part $\phi''$ depending on the other $k-d-1$ variables.
For a fixed
we can then regard
As in the proof of Theorem \ref{thm:main}, we can use the triangle inequality and obtain the bound
$$\|\Gamma^{\phi}_f\|_{\square^{k}_{d}} \leq \max_{a \in G} \|\Gamma^{\phi'}_{T^a f}\|_{\square^{d+1}_d}.$$
Now the desired inequality follows from the already considered case $k=d+1$ for the form~$\phi'$.


\medskip
$(ii)$
We first show that $\|\Gamma^{(k)}_f\|_{\square^k_d} \leq \max_{a \in G} \|\Gamma^{\phi}_{T^a f}\|_{\square^k_d}$ always holds.
Denote $\phi(x_1, \dots, x_k) = \lambda_1 x_1 + \dots + \lambda_k x_k$, and for each $1 \leq i \leq k$ fix a set $R_i \subseteq G$ of representatives of $G/\lambda_i G$.
Note that, if $r$ is uniformly distributed over~$R_i$ and~$y$ is uniformly distributed over~$G$, then $r + \lambda_i y$ will be uniformly distributed over~$G$.

Choose optimal functions $u_B: G^B \rightarrow [0, 1]$, $B \in \binom{[k]}{d}$, so that
$$\|\Gamma^{(k)}_f\|_{\square^{k}_{d}} = \Bigg| \mathbb{E}_{\xbf \in G^{k}} \Bigg[ f(x_1 + \dots + x_k) \prod_{B \in \binom{[k]}{d}} u_B(\xbf_B) \Bigg] \Bigg|.$$
Performing the change of variables $x_i = r_i + \lambda_i y_i$ for each $i \in [k]$, we have
\begin{align*}
    \|\Gamma^{(k)}_f\|_{\square^{k}_{d}} = \Bigg| \mathbb{E}_{r_1 \in R_1, \dots, r_k \in R_k} \mathbb{E}_{y_1, \dots, y_k \in G^{k}} \Bigg[ f(x_1 + \dots + x_k) \prod_{B \in \binom{[k]}{d}} u_B(\xbf_B) \Bigg] \Bigg|.
\end{align*}
There must then be some values $r_1 \in R_1$, $\dots$, $r_k \in R_k$ for which
$$\|\Gamma^{(k)}_f\|_{\square^{k}_{d}} \leq
\Bigg| \mathbb{E}_{y_1, \dots, y_k \in G^{k}} \Bigg[ f\bigg( \sum_{i=1}^k (r_i + \lambda_i y_i) \bigg) \prod_{B \in \binom{[k]}{d}} u_B\big( (r_i + \lambda_i y_i)_{i \in B} \big) \Bigg] \Bigg|;$$
given such values, denote $v_B: G^B \rightarrow [0, 1]$ the function given by
$$v_B(\ybf_B) = u_B\big( (r_i + \lambda_i y_i)_{i \in B} \big).$$
We then have
\begin{align*}
    \|\Gamma^{(k)}_f\|_{\square^{k}_{d}}
    &\leq \Bigg| \mathbb{E}_{y_1, \dots, y_k \in G^{k}} \Bigg[ T^{r_1 + \dots + r_k} f\bigg( \sum_{i=1}^k \lambda_i y_i \bigg) \prod_{B \in \binom{[k]}{d}} v_B(\ybf_B) \Bigg] \Bigg| \\
    &\leq \|\Gamma^{\phi}_{T^{r_1 + \dots + r_k} f}\|_{\square^k_d},
\end{align*}
as wished.

Now we note that $\|\Gamma^{\phi}_{T^a f}\|_{\square^k_d} = \|\Gamma^{\phi}_f\|_{\square^k_d}$ for all $a \in G$ if $\phi$ is surjective.
The result now follows from the usual Cayley case.
\end{proof}

The next simple examples show that the conditions on the linear form $\phi$ in each item of the last theorem cannot be dropped:

\begin{ex}
    Let $G = \F_2^n \oplus \F_3^n$ and define the linear form $\phi: G^2 \rightarrow G$ by
    $$\phi(x_1, x_2) = 3x_1 + 2x_2;$$
    this form is clearly surjective.
    Let $R \subset \F_2^n$ be a very linearly uniform set of density $1/2$ (for instance $R$ can be a set of $2^{n-1}$ elements of $\F_2^n$ chosen uniformly at random),
    and consider the set
    $$A := R \oplus \F_3^n = \{(x, y) \in \F_2^n \oplus \F_3^n:\, x\in R\}$$
    This set has density $1/2$, and it is easy to see that $3x_1 + 2x_2 \in A$ if and only if $x_1 \in A$.
    The hypergraph $\Gamma^{\phi}_A$ will then have edge density $1/2$ and
    $$\|\Gamma^{\phi}_A - 1/2\|_{\square^2_1} \geq
    \mathbb{E}_{x_1, x_2 \in G}\left[ \left(A(3x_1 + 2x_2) - 1/2\right) A(x_1) \right] = 1/4;$$
    $\Gamma^{\phi}_A$ is therefore \emph{not} quasirandom of order $1$.
    
    We now compute the Fourier coefficients of $A$, which measure how linearly uniform the set $A$ is.
    Any character $\gamma \in \widehat{G}$ can be decomposed as $\gamma = \gamma_1 \cdot \gamma_2$ for some $\gamma_1 \in \widehat{\F_2^n}$ and $\gamma_2 \in \widehat{\F_3^n}$.
    Then
    \begin{align*}
        |\widehat{A}(\gamma)|
        &= \left|\mathbb{E}_{(x, y) \in \F_2^n \oplus \F_3^n}\left[ A\left((x, y)\right) \overline{\gamma_1(x)} \overline{\gamma_2(y)} \right]\right| \\
        &= \left|\mathbb{E}_{x \in \F_2^n}\left[ R(x) \gamma_1(x) \right]\right| \left|\mathbb{E}_{y \in \F_3^n}\left[ \gamma_2(y) \right]\right|
    \end{align*}
    If $\gamma_2$ is \emph{not} the trivial character $\mathbf{1}$, then this last expression is zero.
    If $\gamma_2 = \mathbf{1}$ then it is $|\widehat{R}(\gamma_1)|$, which by uniformity of $R$ will be $o(1)$ whenever $\gamma_1 \neq \mathbf{1}$.
    Thus $|\widehat{A}(\gamma)| = o(1)$ whenever $\gamma$ is a non-trivial character, showing that $A$ is very linearly uniform.
    
    This example can be easily generalized to any edge-size $k \geq 2$ of the hypergraph $\Gamma^{\phi}_A$ in consideration.
    For instance, we can instead consider the group $G = \F_2^n \oplus \F_3^n \oplus \F_5^n$ and the surjective linear form $\phi: G^3 \rightarrow G$ given by
    $$\phi(x_1, x_2, x_3) = 3 \cdot 5 x_1 + 2 \cdot 5 x_2 + 2 \cdot 3 x_3$$
    Taking again a linearly uniform set $R \subset \F_2^n$ of density $1/2$ and defining
    $$A := R \oplus \F_3^n \oplus \F_5^n = \{(x, y, z) \in \F_2^n \oplus \F_3^n \oplus \F_5^n:\, x\in R\}$$
    we conclude by the same argument that $A$ is linearly uniform in $G$ but $\Gamma^{\phi}_A$ is not quasirandom of order $1$ since
    $$\|\Gamma^{\phi}_A - 1/2\|_{\square_1^3} \geq \mathbb{E}_{x_1, x_2, x_3 \in G}\left[ \left(A(\phi(x_1, x_2, x_3)) - 1/2\right) A(x_1) \right] = 1/4$$
\end{ex}

\begin{ex}
    Let $G = \F_2 \oplus \Z_N$ where $N$ is a large odd integer, and define the linear form $\phi: G^d \rightarrow G$ by
    $$\phi(x_1, x_2, \dots, x_d) = 2x_1 + 2x_2 + \dots + 2x_d$$
    This form is not surjective, but the subgroup $2G$ is quite `large': $|2G|/|G| = 1/2$.
    Take a set $R \subset \Z_N$ which is very uniform of degree $d-1$, and consider
    $$A := \{0\} \oplus 2R = \{(0, 2y) \in \F_2 \oplus \Z_N:\, y \in R\}$$
    The hypergraph $\Gamma^{\phi}_A$ will have the same density as $R$ and will be quasirandom of order $d-1$, but since $A$ is concentrated on the subgroup $\{0\} \oplus \Z_N$ it will \emph{not} be uniform of degree $d-1$ (or even linearly uniform).
    
    In general, whenever $G$ is an additive group and $\phi: G^d \rightarrow G$ is not surjective, we have $|\phi(G^d)|/|G| \leq 1/2$.
    Given any set $A \subseteq G$ the hypergraph $\Gamma^{\phi}_A$ will depend only on $A \cap \phi(G^d)$, and we can break any uniformity of the set $A$ by either adding to or removing from $A$ all elements in $G \setminus \phi(G^d)$, which does not impact the quasirandomness of $\Gamma^{\phi}_A$.
\end{ex}

The simplest and most common way of dealing with these divisibility issues is by requiring all coefficients of the linear form $\phi$ considered to be coprime to the size $|G|$ of the group;
if this happens we say that $\phi$ is \emph{coprime}.
For such linear forms we obtain in item $(i)$ that $\Gamma^{\phi}_A$ is $\varepsilon$-quasirandom of order $d-1$ whenever $A$ is $\varepsilon$-uniform of degree $d-1$;
in item $(ii)$ we obtain that $A$ is $2 \varepsilon^{1/2^d}$-uniform of degree $d-1$ whenever $\Gamma^{\phi}_A$ is $\varepsilon$-quasirandom of order $d-1$.

The next theorem easily follows from the same arguments used for proving Theorem~\ref{Cayley_equiv}.
%and the observation that $x \mapsto \lambda x$ is a bijection if $\gcd(\lambda, |G|) = 1$.

\begin{thm}%[Equivalence theorem for quasirandom Cayley hypergraphs] \label{Cayley_equiv}
%Let $d \geq 1$ be an integer, and let $A \subseteq G$ be a set of density $\delta$ in $G$.
%Then for every fixed $k \geq d+1$ the following statements are polynomially equivalent:
Let $d \geq 1$ be an integer and~$k\geq d+1$.
For every coprime form $\phi: G^k \to G$ the following statements are polynomially equivalent, where $G$ is a finite additive group and $A \subseteq G$ is a subset of density $\delta$:
\begin{itemize}
    \item[$(i)$] $A$ is uniform of degree $d$:\quad
    $\| A - \delta \|_{U^{d+1}} \leq c_1$.
    \item[$(ii)$] $A$ has few patterns of type $\Phi^{(k)}_d$:
    $$\mathbb{P}_{\xbf \in G^{V(k, d)}}\big( \Phi^{(k)}_d(\xbf) \subseteq A \big) \leq \delta^{2^{\binom{k}{d}}} + c_2.$$
    \item[$(iii)$] $\Gamma^{\phi}_A$ is quasirandom of order $d$:\quad
    $\| \Gamma^{\phi}_A - \delta \|_{\square^k_d} \leq c_3$.
    \item[$(iv)$] $\Gamma^{(k)}_A$ correctly counts all $k$-partite $d$-linear hypergraphs:
    $$t_{can}(F,\, \Gamma^{\phi}_A) = \delta^{|F|} \pm c_4 |F| \quad \text{for all $F \in \mathcal{L}^{(k)}_{d}$ $k$-partite}.$$
    \item[$(v)$] $\Gamma^{(k)}_A$ correctly counts all $k$-partite $(d+1)$-simple hypergraphs:
    $$t_{can}(F,\, \Gamma^{\phi}_A) = \delta^{|F|} \pm c_5 |F| \quad \text{for all $F \in \mathcal{S}^{(k)}_{d+1}$ $k$-partite}.$$
    \item[$(vi)$] $\Gamma^{\phi}_A$ has few squashed octahedra $\oct^{(k)}_{d+1}$:
    $$t_{can}\big( \oct^{(k)}_{d+1},\, \Gamma^{\phi}_A \big) \leq \delta^{2^{d+1}} + c_6.$$
    \item[$(vii)$] $\Gamma^{\phi}_A$ has small $(d+1)$-deviation:
    \quad $\dev_{d+1}\big(\Gamma^{\phi}_A\big) \leq c_7$.
\end{itemize}
\end{thm}

\begin{proof}
Since $x \mapsto \lambda x$ is a bijection if $\gcd(\lambda, |G|) = 1$, it follows that $\Gamma^{\phi}_A$ is isomorphic to $H_s A$
(that is, the $k$-partite hypergraph induced by the `sum' linear form $\Sigma(x_1, \dots, x_k) = x_1 + \dots +x_k$).
The result then follows from the same arguments used to prove Theorem \ref{Cayley_equiv}, using the partite version of the strongly quasirandom theorem for hypergraphs.
\end{proof}


\subsection{Quasirandomness from counting $s$-simple hypergraphs} \label{NewQuasirandomSection}

We have seen in the last theorem that Cayley hypergraphs of sets which are uniform of degree $s-1$ contain the expected number of all $s$-simple hypergraphs, even though they are only guaranteed to be quasirandom of order $s-1$.

Say something about what the notion of hypergraph quasirandomness corresponds to uniformity of degree $d$.

The ability to count all hypergraphs in $\mathcal{S}^{(k)}_{d}$ is due to some extra symmetries satisfied by Cayley hypergraphs.
It can be shown that these (approximate) symmetries are in fact \emph{necessary and sufficient} for a large hypergraph to have the `correct' count of all $d$-simple hypergraphs, or even only of $\oct^{(k)}_{d}$.

In fact, Cayley hypergraphs have the property that all its link hypergraphs are very similar to each other;
if $A$ is uniform of some degree $d$, then these link hypergraphs will all behave the same

Such a result can be seen as giving rise to a distinct notion of quasirandomness for hypergraphs. (Define the link hypergraph $H_{\ybf}$)

We note that Gowers and Wolf \cite{TrueComplexity} noted
noticed something similar to:
the corresponding notion of uniformity of some degree $d$ for hypergraphs would allow one to control the count of $d$-simple hypergraphs.
$\varrho, \varsigma$

\begin{thm}
Let $1 \leq s \leq k$ be integers and let $H$ be a $k$-uniform hypergraph with edge density $\delta$.
Then the following properties are polynomially equivalent:
\begin{itemize}
    \item[$(i)$] $H$ is $c_1$-quasirandom of order $s-1$,
    and almost all link $s$-graphs are similar to each other:
    $$\|H_{\ybf} - H_{\mathbf{y'}}\|_{\square^s_{s-1}} \leq c_1 \quad \text{for all but at most $c_1 v(H)^{2(k-s)}$ pairs } \ybf, \mathbf{y'} \in V^{k-s}.$$
    %and for all but at most $c_1' v(H)^{2(k-d-1)}$ pairs $\ybf, \mathbf{y'} \in V^{k-d-1}$ we have $\|H_{\ybf} - H_{\mathbf{y'}}\|_{\square^{d+1}_{d}} \leq c_1'$.
    \item[$(ii)$] For all but at most $c_2 v(H)^{k-s}$ tuples $\ybf \in V^{k-s}$ the link $s$-graph $H_{\ybf}$ is $c_2$-quasirandom of order $s-1$.
    %and has edge density $\delta \pm c_1$.
    \item[$(iii)$] $H$ correctly counts all $s$-simple hypergraphs:
    $$t(F,\, H) = \delta^{|F|} \pm |F|c_3 \hspace{5mm} \forall F \in \mathcal{S}^{(k)}_{s}.$$
    \item[$(iv)$] $H$ has few squashed octahedra $\oct^{(k)}_{s}$: \quad
    $t(\oct^{(k)}_{s},\, H) \leq \delta^{2^s} + c_4$.
    \item[$(v)$] $H$ has small $s$-deviation: \quad
    $\dev_s(H) \leq c_5$.
    %$$\hspace{-1cm} \mathbb{E}_{\xbf^{(0)}, \xbf^{(1)} \in V^s} \mathbb{E}_{y_{s+1}, \dots, y_k \in V} \Bigg[ \prod_{\omega \in \{0, 1\}^s} \big( H(x_1^{(\omega_1)}, \dots, x_{s}^{(\omega_{s})}, y_{s+1}, \dots, y_k) - \delta \big) \Bigg] \leq c_5.$$
\end{itemize}
\end{thm}

Note that when $d = 1$ the condition of `quasirandomness of order 0' in the first item is trivially satisfied, and when $d = k$ we obtain this result is equivalent to some Theorem on strongly quasirandom properties of hypergraphs.

It is perhaps appropriate to remark that item $(i)$ is more stringent than it might first appear:
we require that most link $d$-graphs are similar as \emph{labeled hypergraphs}, not only that they are similar up to isomorphism.
By the theorem, this strong property is forced on $H$ whenever one of the other items are satisfied, but it is likely only because the link hypergraphs are similar to the constant $\delta$ function which is invariant under relabeling.
If one can substitute the cut norm for cut distance then this would provide a (likely much simpler) proof of Theorem \ref{thm:main}.

Another interesting thing to remark is that item $(ii)$ requires only that the link $d$-graphs be quasirandom, but makes no assumption on the original hypergraph $H$ or even on what the densities of each link hypergraph are.
It will follow from the proof that this seemingly weak property already implies that $H$ itself is quasirandom and that most densities of link $d$-graphs are very close to the density of $H$, but this is not assumed a priori.

\begin{proof}
$(i) \Rightarrow (ii)$:
Suppose the vertex set of $F$ is $[\ell]$ and write $F = \{e_1, \dots, e_{|F|}\}$.
Proceeding as in the proof of Theorem \ref{Cayley_equiv}, we obtain that
$$\left| t(F, H) - \delta^{|F|} \right| \,\leq\, \sum_{i = 1}^{|F|} \mathbb{E}_{\xbf_{[\ell] \setminus f_i}} \left|\mathbb{E}_{\xbf_{f_i}} \left[ \left( H(\xbf_{e_i}) - \delta \right) \prod_{j = i+1}^{|F|}{H(\xbf_{e_j})} \right]\right|$$
where each $f_i \subseteq e_i$ is a set of $d$ vertices in $F$ which is not completely contained in any other edge of $F$.

Let us consider the $i$-th term in the last sum.
For a fixed $\xbf_{[\ell] \setminus f_i} \in V^{[\ell] \setminus f_i}$ and each $i+1 \leq j \leq |F|$, define the function $u_{j, \xbf_{[\ell] \setminus f_i}}$ on $V^{e_j \cap f_i}$ by $u_{j, \xbf_{[\ell] \setminus f_i}}(\xbf_{e_j \cap f_i}) = H(\xbf_{e_j})$.
Since $|e_j \cap f_i| \leq d-1$ for $j \neq i$, the last sum is
\begin{align*}
    \sum_{i = 1}^{|F|} \mathbb{E}_{\xbf_{[\ell] \setminus f_i}} &\left|\mathbb{E}_{\xbf_{f_i}} \left[ \left(H_{\xbf_{e_i \setminus f_i}}(\xbf_{f_i}) - \delta\right) \prod_{j = i+1}^{|F|}{u_{j, \xbf_{[\ell] \setminus f_i}}(\xbf_{e_j \cap f_i})} \right]\right| \\
    &\hspace{3cm} \leq \sum_{i = 1}^{|F|} \mathbb{E}_{\xbf_{[\ell] \setminus f_i}} \| H_{\xbf_{e_i \setminus f_i}} - \delta \|_{\square^d_{d-1}} \\
    &\hspace{3cm} = |F| \cdot \mathbb{E}_{\ybf \in V^{k-d}} \left\| H_{\ybf} - \delta \right\|_{\square^d_{d-1}}
\end{align*}
From the condition in item $(i)$ we have
$\mathbb{E}_{\ybf \in V^{k-d}} \left\| H_{\ybf} - \delta \right\|_{\square^d_{d-1}} \leq 3c_1$,
so we obtain item $(ii)$ with $c_2 = 3c_1$.

\medskip
$(ii) \Rightarrow (iii)$:
This is a special case, and we may take $c_3 = 2^{d}c_2$.

\medskip
$(iii) \Rightarrow (iv)$:
We first note that
\begin{align*}
    t(\oct^{(k)}_{d}, H) \,&=\, \mathbb{E}_{\ybf \in V^{k-d}} \mathbb{E}_{\xbf^{(0)}, \xbf^{(1)} \in V^{d}} \left[ \prod_{\omega \in \{0, 1\}^{d}} H(\xbf^{(\omega)}, \ybf) \right] \\
    &=\, \mathbb{E}_{\ybf \in V^{k-d}} \left[ t(\oct^{(d)}, H_{\ybf}) \right]
\end{align*}
We are then given that $\mathbb{E}_{\ybf \in V^{k-d}}\left[ t(\oct^{(d)}, H_{\ybf}) \right] \leq \delta^{2^d} + c_3$ and we wish to bound the expression
$\mathbb{E}_{\ybf \in V^{k-d}}\left[ t(\oct^{(d)}, H_{\ybf} - \delta) \right]$.

Fix some tuple $\ybf \in V^{k-d}$.
As in the case of Cayley hypergraphs, we shall consider the expression
$$t(\oct^{(d)}, H_{\ybf} + \delta) + t(\oct^{(d)}, H_{\ybf} - \delta) = \sum_{F \subseteq \oct^{(d)}} t(F, H_{\ybf}) \left( \delta^{2^d-|F|} + (-\delta)^{2^d-|F|} \right)$$
By Gowers-Cauchy-Schwarz we have that $t(F, H_{\ybf}) \leq \|H_{\ybf}\|_{\oct^k}^{|F|}$ holds for all subhypergraphs $F \subseteq \oct^{(d)}$, and so
$$t(\oct^{(d)}, H_{\ybf} + \delta) + t(\oct^{(d)}, H_{\ybf} - \delta) \leq \sum_{F \subseteq \oct^{(d)}} \|H_{\ybf}\|_{\oct^d}^{|F|} \left( \delta^{2^d - |F|} + (-\delta)^{2^d - |F|} \right)$$

Taking the expectation over all $\ybf \in V^{k-d}$ and then using convexity, we conclude
\begin{align*}
    \mathbb{E}_{\ybf}\left[ t(\oct^{(d)}, H_{\ybf} + \delta)\right. &+ \left. t(\oct^{(d)}, H_{\ybf} - \delta) \right] \\
    &\leq \sum_{F \subseteq \oct^{(d)}} \mathbb{E}_{\ybf} \left[\|H_{\ybf}\|_{\oct^d}^{|F|}\right] \left( \delta^{2^d - |F|} + (-\delta)^{2^d - |F|} \right) \\
    &\leq \sum_{F \subseteq \oct^{(d)}} \mathbb{E}_{\ybf} \left[\|H_{\ybf}\|_{\oct^d}^{2^d}\right]^{|F|/2^d} \left( \delta^{2^d - |F|} + (-\delta)^{2^d - |F|} \right) \\
    &= \left( \mathbb{E}_{\ybf} \left[\|H_{\ybf}\|_{\oct^d}^{2^d}\right]^{1/2^d} + \delta \right)^{2^d} + \left( \mathbb{E}_{\ybf} \left[\|H_{\ybf}\|_{\oct^d}^{2^d}\right]^{1/2^d} - \delta \right)^{2^d}
\end{align*}
where the last equality follows from the binomial expansion.

Let us denote the edge density of each link hypergraph $H_{\ybf}$ by $\delta_{\ybf}$;
it is clear that $\mathbb{E}_{\ybf \in V^{k-d}} [\delta_{\ybf}] = \delta$.
Using convexity and our assumption from item $(iii)$ we have that
$$\delta \leq \mathbb{E}_{\ybf} \left[\delta_{\ybf}^{2^d}\right]^{1/2^d} \leq \mathbb{E}_{\ybf} \left[\|H_{\ybf}\|_{\oct^d}^{2^d}\right]^{1/2^d} \leq \delta + c_3^{1/2^d}$$
and
$$\mathbb{E}_{\ybf} \left[t(\oct^{(d)}, H_{\ybf} + \delta)\right] = \mathbb{E}_{\ybf} \left[\|H_{\ybf} + \delta\|_{\oct^d}^{2^d}\right] \geq \mathbb{E}_{\ybf} \left[(\delta_{\ybf} + \delta)^{2^d}\right] \geq (2\delta)^{2^d}$$
We thus obtain from our earlier estimate that
$$\mathbb{E}_{\ybf} \left[t(\oct^{(d)}, H_{\ybf} - \delta)\right] + (2\delta)^{2^d} \leq \left( 2\delta + c_3^{1/2^d} \right)^{2^d} + c_3,$$
which by a simple computation implies
$$t(\oct^{(k)}_{d}, H - \delta) = \mathbb{E}_{\ybf} \left[t(\oct^{(d)}, H_{\ybf} - \delta)\right] \leq 2^{2^{d+1}} c_3^{1/2^d}$$
This is exactly item $(iv)$ with constant $c_4 = 2^{2^{d+1}} c_3^{1/2^d}$.


\medskip
$(iv) \Rightarrow (i)$:
As noted before, the $d$-deviation of $H$ can be written as
$$t(\oct^{(k)}_{d}, H - \delta) = \mathbb{E}_{\ybf \in V^{k-d}} \left[t(\oct^{(d)}, H_{\ybf} - \delta)\right] = \mathbb{E}_{\ybf \in V^{k-d}} \left[ \|H_{\ybf} - \delta\|_{\oct^d}^{2^d} \right]$$
If this is at most $c_4$, then at most $c_4^{1/2} |V|^{k-d}$ tuples $\ybf \in V^{k-d}$ can satisfy the inequality $\|H_{\ybf} - \delta\|_{\oct^d}^{2^d} \geq c_4^{1/2}$.
For all other choices of $\ybf \in V^{k-d}$ we have
$$\|H_{\ybf} - \delta\|_{\square^d_{d-1}} \leq \|H_{\ybf} - \delta\|_{\oct^d} \leq c_4^{1/2^{d}}$$
(where we have used Lemma \ref{lem:cut<oct} for the first inequality);
this implies item $(i)$ with constant $c_1 = c_4^{1/2^{d}}$.
\end{proof}

We remark that a similar result can be also obtained
%such a result also follows
from the main theorem of Towsner \cite{SigmaAlgebrasHypergraphs}, when considering the collection $\mathcal{I} = \left\{S \in \binom{k}{k-1}:\, [d] \subseteq S \right\}$.


\subsection{Limitations of the hypergraph approach to uniformity}


